UniPROT: Uniform Prototype Selection via Partial Optimal Transport with Submodular Guarantees

Selecting prototypical examples from a source distribution to represent a target data distribution is a fundamental problem in machine learning. Existing subset selection methods often rely on implicit importance scores, which can be skewed towards majority classes and lead to low-quality prototypes for minority classes. We present $\methodprop$, a novel subset selection framework that minimizes the optimal transport (OT) distance between a uniformly weighted prototypical distribution and the target distribution. While intuitive, this formulation leads to a cardinality-constrained maximization of a \emph{super-additive} objective, which is generally intractable to approximate efficiently. To address this, we propose a principled reformulation of the OT marginal constraints, yielding a partial optimal transport-based submodular objective. We prove that this reformulation enables a greedy algorithm with a $(1-1/e)$ approximation guarantee relative to the original super-additive maximization problem. Empirically, we showcase that enforcing uniform prototype weights in UniPROT consistently improves minority-class representation in imbalanced classification benchmarks without compromising majority-class accuracy. In both finetuning and pretraining regimes for large language models under domain imbalance, UniPROT enforces uniform source contributions, yielding robust performance gains. Our results establish UniPROT as a scalable, theoretically grounded solution for uniform-weighted prototype selection. Our code is publicly available at GitHub\footnote{Code: https://github.com/efficiency-learning/UniPROT}

==> ExperimentsPlots/SpotGreedyMotivation/spotgreedy_motivation.tex <==
% This file was created with tikzplotlib v0.10.1.
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{groupplot}[group style={group size=5 by 2}, height=2cm, width=2cm, title style={font=\bfseries\large}, title shift=0.5cm]
\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={1
0.14},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-000.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={2
0.13},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-001.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={3
0.12},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-002.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={4
0.11},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-003.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={5
0.10},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-004.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={6
0.10},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-005.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={7
0.09},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-006.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={8
0.08},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-007.png};

\nextgroupplot[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
title={9
0.07},
x grid style={darkgray176},
xmin=-0.5, xmax=27.5,
xtick style={color=black},
xtick={-25,0,25,50},
xticklabels={
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {0}\),
  \(\displaystyle {25}\),
  \(\displaystyle {50}\)
},
y dir=reverse,
y grid style={darkgray176},
ymin=-0.5, ymax=27.5,
ytick style={color=black},
ytick={-20,0,20,40},
yticklabels={
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {0}\),
  \(\displaystyle {20}\),
  \(\displaystyle {40}\)
}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {ExperimentsPlots/SpotGreedyMotivation/spotgreedy_mnist_ranked_medoids-009.png};
\end{groupplot}

\draw ({$(current bounding box.south west)!0.5!(current bounding box.south east)$}|-{$(current bounding box.south west)!0.98!(current bounding box.north west)$}) node[
  scale=0.8,
  anchor=north,
  text=black,
  rotate=0.0
]{\bfseries SpotGreedy MNIST Medoids Ranked by Weights};
\end{tikzpicture}


==> iclr2026/applications.tex <==
\section{Real World Applications}

\textbf{Gradient Matching}
Validation aware gradient matching
\citep{gradmatch} and \citep{greats}

and \citep{minibatchcoresets}

\subsection{Application: Validation-Aware Online Data Selection via Fair Entropic POT}

Let $\mathcal{D} = \{(\bx_i, y_i)\}_{i=1}^n$ denote the training dataset for a classification task. At iteration $t$, we consider a candidate batch $B_t \subset \mathcal{D}$ and a validation instance $z_{\text{val}} = (\bx_{\text{val}}, y_{\text{val}})$. We wish to select a subset $\mathcal{P} \subseteq B_t$ of size $k$ to perform a model update that maximally reduces the validation loss.

Define the virtual model update rule:
\[
w_{t+1}(\mathcal{P}) := \bw_t - \eta_t \sum_{z \in \mathcal{P}} \nabla \ell(\bw_t, z)
\]
and the utility of a candidate subset $\mathcal{P}$ as the reduction in validation loss:
\[
U^{(t)}(\mathcal{P}; z_{\text{val}}) := \ell(\bw_t, z_{\text{val}}) - \ell(w_{t+1}(\mathcal{P}), z_{\text{val}})
\]

Since directly computing this is expensive, a first-order Taylor approximation yields the marginal gain for adding a point $z_i \in B_t$ (given a fixed selection $\mathcal{P}$):
\[
U^{(t)}(z_i \mid \mathcal{P}) \approx \eta_t \left\langle \nabla \ell(\bw_t, z_i), \nabla \ell(w_{t+1}(\mathcal{P}), z_{\text{val}}) \right\rangle
\]

The gradient $\nabla \ell(w_{t+1}(\mathcal{P}), z_{\text{val}})$ is itself approximated via:
\[
\nabla \ell(w_{t+1}(\mathcal{P}), z_{\text{val}}) \approx \nabla \ell(\bw_t, z_{\text{val}}) - \eta_t H(z_{\text{val}}) \sum_{z \in \mathcal{P}} \nabla \ell(\bw_t, z)
\]
where $H(z_{\text{val}}) := \nabla^2 \ell(\bw_t, z_{\text{val}})$ is the Hessian.

Substituting, we obtain:
\[
U^{(t)}(z_i \mid \mathcal{P}) \approx \eta_t \left\langle \nabla \ell(\bw_t, z_i), \nabla \ell(\bw_t, z_{\text{val}}) \right\rangle - \eta_t^2 \nabla \ell(\bw_t, z_i)^\top H(z_{\text{val}}) \sum_{z \in \mathcal{P}} \nabla \ell(\bw_t, z)
\]

We now reframe this selection problem as a Fair Entropic Partial Optimal Transport(POT) objective:

\paragraph{Reformulation as Fair Entropic POT.} Let $G \in \mathbb{R}^{d \times |B_t|}$ be the matrix of gradients $\nabla \ell(\bw_t, z_i)$ for $z_i \in B_t$, and let $g_{\text{val}} := \nabla \ell(\bw_t, z_{\text{val}})$. Define a similarity matrix $\mathbb{S} \in \mathbb{R}^{|B_t| \times 1}$ with:
\[
\mathbb{S}_{i} := \left\langle \nabla \ell(\bw_t, z_i), g_{\text{val}} \right\rangle
\]

We seek to select a subset $\mathcal{P} \subseteq B_t$ of size $k$, and define an entropic regularized transport plan $\mgamma \in \mathbb{R}_+^{k \times 1}$ with uniform source marginals:
\[
\mgamma^\top \mathbf{1} = 1, \quad \mgamma_i \geq 0
\]

The resulting fair OT objective becomes:
\[
f(\mathcal{P}) := \max_{\mgamma \in \mathbb{R}_+^{k \times 1}, \ \mgamma^\top \mathbf{1} = 1} \left[ \left\langle \mathbb{S}_{\mathcal{P}}, \mgamma \right\rangle + \lambda H(\mgamma) \right]
\]
where $H(\mgamma) := - \sum_{i=1}^k \mgamma_i \log \mgamma_i$ denotes the entropy.

\paragraph{Interpretation.} This formulation interprets validation-aware batch selection as transporting training gradients (from selected samples) to match the validation gradient direction. 



\textbf{PU Learning}

\textbf{Fair MLC}

==> iclr2026/extras.tex <==

    Let $\S:= \{\bx_{i}\}_{i=1}^{m}$ and $\T:= \{\by_{j}\}_{j=1}^{n}$ be i.i.d
    samples from source and target distribution $\mathbb{S}$ and $\mathbb{T}$, respectively.
    We assume we have access to the empirical distributions as
    $\mathbb{S}= \sum_{i=1}^{m}{\bmu_S}_{i}\delta_{x_i}$; $\mathbb{T}= \sum_{j=1}
    ^{n}{\bnu_{\bT}}_{j}\delta_{y_j}$ where the probabilities associated with sample $\bx_{i}$ and $\by_{j}$ are
    ${\bmu_S}_{i}$ and ${\bnu_{\bT}}_{j}$ respectively and $\delta$ is the Dirac
    delta function.


\[\Function{POT}{$\P$, $k$, $\widetilde{\sS}$, $\bmu_{\P}$, $\bmu_{\sT}$}
%\Require Vectors $\bmu_{\bS} \in \RR^m_{\geq 0}$, $\bnu_{\bT} \in \RR^n_{\geq 0}$, cost matrix $\bC \in \RR^{m \times n}$, regularization $\lambda > 0$, tolerance $\epsilon$
\Statex \hspace*{1em} \texttt{// Compute entropic transport via Sinkhorn}
\Statex \hspace*{1em} Compute Gibbs kernel: $\bK \gets \exp(-\lambda \bC)$ \Comment{Elementwise exponentiation}
\Statex \hspace*{1em} Initialize: $\bu^{(0)} \gets \bone_m$, $\bv^{(0)} \gets \bone_n$
\For{$t = 1$ to max iterations}
    \Statex \hspace*{2em} $\bu^{(t)} \gets \bmu_{P} \oslash (\bK \bv^{(t-1)})$ \Comment{Elementwise division}
    \Statex \hspace*{2em} $\bv^{(t)} \gets \bmu_{T} \oslash (\bK^\top \bu^{(t)})$
    \If{converged: $\|\bu^{(t)} \odot (\bK \bv^{(t)}) - \bmu_{P}\|_1 < \epsilon$ \\ 
    \hspace*{6em} and $\|\bv^{(t)} \odot (\bK^\top \bu^{(t)}) - \bmu_{T}\|_1 < \epsilon$}
        \Statex \hspace*{2em} \textbf{break}
    \EndIf
\EndFor
\Statex \hspace*{1em} \Return $\mgamma_{\P}^\ast \gets \diag(\bu^{(t)}) \cdot \bK \cdot \diag(\bv^{(t)})$
\EndFunction\]

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{amsthm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak




% Define the lemma environment, BM:
\newtheorem{lemma}{Lemma}

% Optional: Define a restated lemma environment, BM:
\newtheorem*{restatelemma}{Restated Lemma}

==> iclr2026/plots/plot_bs16_phi2_colm.tex <==
0 1.331
1 1.329935
4 1.33041165
5 1.3287685335
8 1.328056848165
9 1.32980027968335
12 1.3284202768865165
14 1.3281020741176515
15 1.3263610533764751
17 1.3258314428427105
19 1.3233591284142834
22 1.3195045371301406
23 1.316450491758839
25 1.3126739868412507
27 1.310231246972838
30 1.3075459345031095
31 1.3039564751580786
34 1.3017039104064978
35 1.297419871302433
38 1.2936636725894086
39 1.2882580358635145
42 1.2844124555048793
44 1.2798433309498305
46 1.2769828976403321
48 1.2721530686639289
50 1.2683625379772896
52 1.2630569125975168
53 1.2590013434715417
56 1.2525903300368262
57 1.248869426736458
60 1.2430467324690935
61 1.2384192651444026
64 1.2343340724929586
65 1.229115731768029
67 1.2233935744503488
69 1.2186986387058452
72 1.2139776523187866
74 1.2104338757955988
75 1.2061505370376429
77 1.2012180316672663
79 1.1968138513505937
82 1.1916927128370878
83 1.187484785708717
86 1.1840849378516298
87 1.1796610884731136
89 1.1749084775883825
92 1.1710633928124985
93 1.1663687588843734
95 1.1616930712955296
98 1.1585081405825743
99 1.1534180591767484
102 1.150375878584981
104 1.1453231197991312
105 1.1413088886011398
108 1.1373167997151283
110 1.132710631717977
112 1.1296335254007972
113 1.1248841901467892
116 1.1224363482453215
117 1.1187499847628684
120 1.1141904849152398
121 1.1115725800660874
123 1.1076858542654264
126 1.1049949957227723
128 1.1005360457655446
129 1.0977696853078893
131 1.0930039884548106
133 1.0903469485702624
136 1.0864144790845598
138 1.0836343342937143
139 1.079196990950777
142 1.0758220210412692
143 1.0718598008308566
146 1.068496202822548
148 1.0670642407943225
149 1.0631635983863792
151 1.0604939624025154
154 1.0567020227784902
155 1.0542240025507053
157 1.0521187625251982
159 1.0475145748999461
161 1.0456094291509466
163 1.042268334859437
165 1.0385846515108428
168 1.0360178049957343
169 1.0325296269457769
171 1.0297283306763192
174 1.025912047369556
175 1.0222089268958605
177 1.0191348376269018
179 1.0183614892506327
181 1.0146518743581265
183 1.0126693556145454
186 1.0094336620584
187 1.006916325437816
190 1.0039821621834377
192 1.0008423405616034
193 0.9972779171559873
195 0.9947921379844274
197 0.9919862166045832
199 0.9898593544385375
201 0.9863367608941521
204 0.9838283932852105
206 0.9805661093523584
207 0.9774934482588349
209 0.9761845137762465
211 0.973297668638484
213 0.9711496919520991
216 0.9663071950325781
217 0.9630561230822523
220 0.9601085618514298
221 0.9578794762329155
224 0.9560746814705863
226 0.9538019346558804
228 0.9507739153093215
229 0.9490021761562283
232 0.9457971543946659
234 0.9437431828507192
235 0.9410827510222121
237 0.93902492351199
240 0.9361766742768701
241 0.9341319075341015
243 0.9312215884587605
246 0.9300403725741728
247 0.9281699688484312
250 0.9250742691599468
251 0.9235795264683474
253 0.9203967312036639
255 0.9189647638916273
257 0.915911116252711
260 0.9151290050901839
262 0.9132957150392821
263 0.9121787578888892
266 0.9114379703100003
268 0.9083975906069003
269 0.9068436147008313
271 0.9056011785538229
273 0.9036101667682847
276 0.9010430651006017
277 0.8993666344495956
279 0.8976059681050997
282 0.8949889084240488
283 0.8930390193398082
285 0.8904746291464101
287 0.889140882854946
290 0.8867384740263965
291 0.8854300892861325
293 0.8831707883932712
296 0.8814290805093385
297 0.8788247897042452
299 0.8770205418072027
302 0.8754873363891307
304 0.8745344630252393
306 0.8718741183949869
307 0.871847377211037
310 0.8696649034389267
311 0.8678792544045374
314 0.8654644618604921
315 0.8646438172418872
318 0.8631643790694684
319 0.8610527352787737
322 0.8593352079259859
323 0.8569748558467262
326 0.856082107288259
328 0.8556912862153764
329 0.8531233733532226
332 0.8531351396196903
334 0.8508627882234935
336 0.8498701603412585
338 0.8475624587378459
339 0.8447868341504674
341 0.8436959658089627
344 0.841522006150873
345 0.8400047860893642
347 0.8391117382284706
350 0.837061620846186
352 0.8348190046377241
354 0.8341108145913468
355 0.8315427064454334
357 0.830855279380979
360 0.8293987265871692
361 0.8288857393212975
364 0.8274778819280846
366 0.8270241031088037
368 0.8246088620777157
370 0.8228867734569385
371 0.8221339057223691
374 0.8215315666651455
375 0.819480250998494
378 0.817404448488509
379 0.8169514040036239
382 0.8162788899635876
383 0.8145791010639517
386 0.8122673100533122
388 0.811518636952779
389 0.8111414505832513
391 0.8108220360774188
394 0.8082008157166446
395 0.8068208075594782
397 0.8044325994838833
399 0.8036542734890445
402 0.8026407307541541
403 0.8022203234466125
405 0.8012201202121464
408 0.7997619190100249
409 0.7974432998199247
412 0.7965258668217254
413 0.7942236081535081
416 0.792154372071973
418 0.7921038283512533
420 0.7914257900677407
421 0.7896745321670633
424 0.7887767868453927
426 0.7864570189769388
428 0.7852404487871694
430 0.7842770442992977
432 0.7828092738563047
434 0.7804071811177417
435 0.7795271093065643
438 0.7790148382134987
439 0.7780536898313637
441 0.7780751529330501
444 0.7772684014037196
445 0.7773667173896823
448 0.7759460502157856
449 0.7752905897136277
452 0.7741336838164915
453 0.7722573469783266
455 0.7700857735085433
458 0.7706089157734579
460 0.7697498266157233
461 0.7708103283495661
463 0.7694842250660704
465 0.7697033828154096
467 0.7678323489872555
470 0.765930025497383
471 0.7651557252424092
473 0.765224167989985
475 0.7639489263100852
478 0.7619384370469843
479 0.7596710526765145
482 0.7592183421497494
484 0.7594461587282519
485 0.7589446971409695
487 0.7585872501695597
490 0.7576043776678641
492 0.7559073338911855
493 0.7544952605522737
495 0.7524093079467509
498 0.7502722148672833
499 0.7509044927186105
502 0.7491844477914245
503 0.7490816033135101
505 0.7485947872803751
508 0.7467998394075713
510 0.7462918410134955
512 0.7463409226033606
514 0.744642513377327
517 0.7445270882435537
518 0.7435618173611183
520 0.7425321991875071
523 0.742569877195632
524 0.7407941784236758
527 0.7392682366394391
529 0.7398135542730447
530 0.7395954187303142
533 0.7390984645430111
534 0.739925479897581
537 0.7388082250986051
538 0.738207142847619
541 0.7369210714191428
543 0.7357808607049514
544 0.736111052097902
546 0.735270941576923
548 0.7348802321611537
551 0.7332684298395422
552 0.7331217455411468
555 0.7314225280857354
557 0.7309633028048781
559 0.7293836697768293
560 0.729783833079061
563 0.7286179947482705
564 0.7288078148007878
567 0.7292087366527799
569 0.7279616492862521
571 0.7278140327933895
573 0.7281798924654556
574 0.7267140935408011
576 0.7265489526053931
578 0.7255034630793391
580 0.7260044284485457
583 0.7246583841640603
584 0.7239358003224197
586 0.7244694423191955
588 0.7234037478960036
590 0.7239617104170436
592 0.7249850933128732
594 0.7247202423797445
597 0.723450039955947
598 0.7219875395563875
600 0.7206716641608236
602 0.7213789475192154
604 0.7203841580440232
606 0.720345316463583
609 0.7190918632989471
611 0.7190399446659577
612 0.7181245452192981
614 0.7182882997671052
616 0.7171414167694342
619 0.7166320026017398
621 0.7148606825757224
622 0.7139740757499652
625 0.7142323349924655
626 0.7126120116425408
629 0.7123928915261154
631 0.7110479626108542
633 0.7119234829847457
635 0.7114312481548983
637 0.7113529356733493
638 0.7118794063166158
640 0.7112076122534496
643 0.7112435361309152
645 0.7096651007696061
647 0.70878744976191
648 0.707665575264291
650 0.707391919511648
652 0.7080170003165316
655 0.7062748303133662
657 0.7055200820102325
658 0.7062778811901301
660 0.7060961023782288
663 0.7052551413544466
664 0.7048905899409021
666 0.7036426840414931
668 0.7033512572010782
671 0.7036827446290673
673 0.7022309171827766
675 0.7007726080109489
677 0.7016238819308394
678 0.701407643111531
680 0.7010045666804158
683 0.7018685210136116
684 0.7013858358034755
686 0.7008319774454407
688 0.7010646576709864
691 0.6999710110942764
693 0.7002803009833336
694 0.6988554979735002
697 0.6976739429937652
699 0.6984152035638275
700 0.6973850515281892
703 0.6966732010129073
705 0.6951964690027782
707 0.6953105043127504
708 0.6938753992696229
710 0.6938116452769266
712 0.6924265288241573
714 0.6916532635359158
716 0.6923227309005566
718 0.6930305035915512
720 0.6905511985556356
722 0.6900646865700792
724 0.6911050397043784
726 0.6906469893073347
729 0.6910105194142614
730 0.6909134142201188
732 0.6929472800779176
734 0.6924158072771385
736 0.6910176492043671
738 0.6916964727123234
740 0.6914915079852002
743 0.6909675929053483
745 0.6906389169762948
747 0.6918545278065318
749 0.6900389825284664
750 0.6892485927031817
752 0.6886341067761499
755 0.6892557657083883
757 0.6887442080513044
758 0.6874137659707914
761 0.6865306283110835
762 0.6865103220279726
764 0.6856242188076928
766 0.6862959766196158
768 0.6855950168534196
770 0.6846840666848854
773 0.6850922260180365
774 0.6868843037578561
776 0.6863614607202775
779 0.6854968461130747
780 0.685039877651944
783 0.6843734788754244
785 0.6844657440866703
787 0.6830050866458035
789 0.6829020357793455
791 0.6816260154215521
792 0.6816457552673365
794 0.6797472977146631
796 0.6799578247375165
799 0.6791232464901413
800 0.6791730140252399
803 0.6799802838849875
805 0.6809984810461377
806 0.6810674962356763
808 0.6801688212733196
810 0.6797641330605864
813 0.6779154917299804
814 0.6765683368126806
817 0.6755726534445539
818 0.6759469269101083
820 0.6751184576410072
822 0.6754952730645971
824 0.6745163203339511
827 0.6747591571306116
829 0.6741455655593055
830 0.6743161099037125
832 0.6736259488046753
835 0.6735436893166286
836 0.6724872524234623
839 0.6721403798992277
841 0.6713489761002354
842 0.6719464863392329
845 0.6708440214758405
847 0.6714225812610822
848 0.6729913554484714
851 0.6724944418939868
853 0.6732354974750469
854 0.6738591425002964
856 0.6735155510752935
858 0.6742033955645405
861 0.673213361608895
862 0.6732512279928061
864 0.672088715712878
867 0.6723448285557492
868 0.6714343802701916
870 0.6717300364674896
872 0.6710967361028147
875 0.6708987687417866
877 0.6717467810543687
879 0.670794313243825
880 0.6714933701113868
882 0.6702954364102729
884 0.6689954820461702
886 0.6698115272257085
888 0.6694124119534515
891 0.669993287833917
893 0.6694403549555779
895 0.669963951406022
897 0.6692233118919618
899 0.6684570787730422
900 0.6689035079853117
902 0.6710454729054587
904 0.6707790181764041
907 0.67228622799464
908 0.6715373657146936
910 0.6716059920575467
913 0.6703519321369712
914 0.6698974128156014
916 0.6704334386874454
918 0.670049104300571
920 0.6688236132575652
922 0.6683373771249896
925 0.6673280033537397
927 0.6680377233202023
928 0.6674843460870002
931 0.6672175026261302
933 0.668317327599869
935 0.6675571543238703
937 0.6671545827806316
938 0.6675440369528253
940 0.667143596583297
942 0.6664411606174641
944 0.6668637490112894
947 0.6667101115211765
949 0.6661470104059648
950 0.6678525403019051
952 0.668197014898886
955 0.6688860447498972
956 0.6676951843023983
959 0.6674312324593743
961 0.6662419201347806
962 0.6656325009334327
965 0.6644181759240984
967 0.6650869941648574
969 0.6646841242232089
971 0.6640292829809767
973 0.6650439901511669
974 0.6648655502496552
977 0.6648568947471586
979 0.664465325799687
981 0.6651566725416901
982 0.6633411058162731
985 0.6636886947581104
986 0.6629648078105292
988 0.662675159732424
990 0.6622554081350996
993 0.6624548540537486
994 0.6613393055132111
997 0.662209912458079
998 0.6620928133334982
1000 0.6602748852001632
1003 0.6611501363481616
1005 0.6596626349846799
1006 0.6590520086348332
1009 0.6587504885484848
1011 0.657764983663
1013 0.6572663338263699
1015 0.6579636704881062
1017 0.6573210337832252
1019 0.6578198234453929
1021 0.657025625210939
1023 0.6564863689588296


==> iclr2026/plots/plot_bs16_phi2_maxloss.tex <==
0 1.3881
1 1.387104
3 1.38820896
5 1.3883418704000001
7 1.390640451696
10 1.39180104717904
12 1.3905370367072496
14 1.3913906663401772
16 1.3899347596767755
17 1.3893804120800077
20 1.3876636079592077
21 1.3867159718796156
24 1.3848728121608194
26 1.3837740840392112
27 1.3818233431988192
29 1.3794221097668309
31 1.3772308886691627
34 1.375804579782471
35 1.3726965339846462
38 1.3709845686448
40 1.3673327229583518
42 1.3642623957287683
44 1.3601977717714806
46 1.358246794053766
47 1.3552293261132282
50 1.3518400328520959
52 1.347479632523575
54 1.3443218361983391
56 1.3395576178363557
57 1.3371700416579921
60 1.3334603412414123
62 1.329170737828998
64 1.3263630304507081
65 1.3226394001462012
67 1.3176630061447392
69 1.3142313760832918
71 1.3102860623224588
73 1.3069542016992342
75 1.3043746596822419
77 1.3001959130854193
80 1.296843953954565
82 1.2929305144150194
83 1.2905132092708693
85 1.2868390771781606
88 1.282925686406379
90 1.2800094295423152
92 1.277109335246892
94 1.2730562418944231
96 1.269888679475479
97 1.265289792680724
100 1.2623918947539168
101 1.2581409758063775
104 1.2541575660483137
106 1.2509449903878305
107 1.2468235404839523
110 1.2429833050791128
111 1.2406074720283218
114 1.2370733973080386
116 1.2349166633349582
117 1.2315364967016087
119 1.2282981317345927
121 1.2261751504172467
124 1.2238563989130742
125 1.2205498349239434
127 1.218782336574704
130 1.2153935132089568
131 1.2128025780768672
134 1.2092945522960985
135 1.2074396067731374
137 1.204644210705406
139 1.200961768598352
142 1.1982691509123684
143 1.1954304594032448
146 1.1930581548092123
148 1.1921075732611202
150 1.188843497528509
152 1.185381062553224
153 1.1831432519276919
156 1.180285819408415
157 1.1780599612143308
159 1.1747483616021874
161 1.1723478779861656
163 1.170102399206304
165 1.166536375214241
168 1.1645040114620986
169 1.1609019713474775
171 1.1589579516340027
174 1.1558113721176626
175 1.153446258396486
177 1.151790795812521
180 1.148955887854396
182 1.147576328975852
183 1.1452275656860935
185 1.1427492900292326
187 1.1411987971289401
189 1.1383808091576506
191 1.136445001066074
193 1.1330275510554133
195 1.1314132755448592
198 1.1285531427894104
199 1.1270916113615164
201 1.1245006952479013
203 1.1215256882954223
205 1.119979431412468
207 1.1171806370983435
209 1.11609883072736
211 1.1130328424200864
213 1.1105915139958855
215 1.1090275988559266
217 1.1066473228673672
219 1.1033188496386936
221 1.1012326611423067
224 1.0989353345308837
225 1.0972729811855748
227 1.096824251373719
230 1.0947140088599818
232 1.0917488687713819
233 1.090025380083668
236 1.0877301262828312
238 1.085278825020003
239 1.0837300367698028
242 1.0814887364021049
243 1.0801298490380837
246 1.078922550547703
247 1.076901325042226
250 1.0743503117918036
251 1.0733078086738856
253 1.0696927305871466
255 1.0689708032812753
257 1.0667580952484625
260 1.066137514295978
262 1.0648031391530182
263 1.0640161077614878
266 1.063439946683873
268 1.0618075472170343
270 1.060307471744864
271 1.0598553970274154
273 1.0580498430571412
276 1.0558793446265697
277 1.054969551180304
279 1.0538608556685012
282 1.0517442471118161
284 1.050441804640698
286 1.0488733865942912
288 1.0470916527283483
289 1.0460997362010647
292 1.044855738839054
293 1.0430561814506634
296 1.0422236196361567
298 1.0404113834397952
299 1.0395502696053973
302 1.0376017669093434
304 1.0367707492402498
306 1.0354290417478473
307 1.0354747513303688
310 1.0335890038170652
311 1.0320671137788946
313 1.0299814426411056
316 1.0286396282146946
317 1.0282252319325478
320 1.0264079796132222
322 1.02533089981709
323 1.023016590818919
325 1.02316042491073
327 1.0211668206616227
329 1.0188341524550064
332 1.0185978109304563
333 1.0166898328211518
336 1.0162629344929404
338 1.0142973051480109
340 1.0131683320965308
341 1.0124166487755655
344 1.01038348228781
346 1.0104956474649318
347 1.0097156909902825
349 1.0086345340803795
352 1.0062421887395758
354 1.00532776685218
355 1.0029734891836581
357 1.0020677542918215
360 1.0005570767489032
362 0.998685505981414
363 0.9983816509215999
366 0.997347834412384
368 0.99492435606826
369 0.9941311125075775
372 0.9944148013825017
373 0.9937956533686767
376 0.9931016968349899
377 0.99117267986664
380 0.9915909530679736
381 0.9902840435372938
383 0.9895092031019209
386 0.9870831110709016
388 0.9867632799601925
390 0.9851616471605906
391 0.9849720306889846
394 0.9826523103820948
396 0.9816857872782738
398 0.980697929405491
400 0.9801449501114361
402 0.9791165006103217
403 0.9786493356042185
406 0.9767928422481763
407 0.9762469138256945
409 0.9736554446874376
412 0.9731648902405632
413 0.9714592413381575
415 0.970880648924776
417 0.9691208424355282
420 0.9688476340111729
421 0.9672461576710611
424 0.9667016960943505
426 0.9650826791334071
428 0.9649978523420729
429 0.9637408738186521
431 0.9635334650804657
434 0.961740130429661
435 0.9608417291253644
438 0.9609663118341107
439 0.9591136487157697
441 0.9593625122286119
443 0.9587318871063258
445 0.9576655682352626
448 0.9562839125529099
449 0.9562200734273808
451 0.955020872693107
454 0.9545056639661759
455 0.9539186073265141
457 0.9529464212532489
459 0.9521819570407164
462 0.9532151374703092
463 0.951931986095606
465 0.95205866623465
468 0.9517200795723035
469 0.9499128787765805
471 0.9489047499888147
473 0.9489877024889266
475 0.9477438254640373
477 0.947089387209397
480 0.945376493337303
482 0.94497672840393
483 0.9441319611198906
486 0.9437556415086917
487 0.9439700850936048
490 0.9435493842426688
491 0.941922890400242
494 0.9416746614962397
495 0.9399799148812773
498 0.9379581157324646
499 0.93847953457514
502 0.9364127392293886
503 0.9366066118370947
506 0.9354765457187237
507 0.9351757802615365
511 0.9343830224589211
512 0.934531192234332
515 0.9342138803119887
517 0.9339737415088689
519 0.9331920040937802
520 0.9315660840528424
523 0.9315604232123139
524 0.9297288189801908
527 0.9281395307903889
529 0.927726135482485
530 0.9273608741276601
532 0.9265062653863835
534 0.9264782027325197
537 0.9255504207051946
539 0.9256709164981427
541 0.9241382073331612
543 0.9230068252598296
544 0.9234847570072313
547 0.922718909437159
548 0.9225207203427873
551 0.9222805131393594
553 0.9205747080079658
554 0.9198849609278861
556 0.9187911113186072
559 0.9182522002054212
560 0.9191266782033669
563 0.9181554114213333
564 0.91831385730712
567 0.9189967187340489
569 0.9185357515467084
571 0.9190433940312412
572 0.9183749600909289
574 0.9169322104900196
576 0.9163198883851195
578 0.9150586895012682
581 0.9155491026062555
583 0.9144196115801929
585 0.914967415464391
586 0.914559741309747
588 0.9128261438966495
590 0.912997882457683
593 0.9121459036331061
594 0.912619444596775
596 0.9117912501508073
599 0.9111563376492993
601 0.9097057742728063
603 0.9102607165300782
604 0.9091271093647775
607 0.9089278382711297
608 0.9082335598884184
611 0.9079532242895342
613 0.9086076920466388
614 0.9084206151261724
616 0.9073014089749107
619 0.9079953948851616
621 0.9061884409363099
622 0.9057735565269468
625 0.9060378209616774
627 0.9048804427520606
628 0.90446163832454
631 0.9030090219412946
633 0.9034079317218817
634 0.902432852404663
636 0.9022885238806163
638 0.9030756386418102
640 0.902025882255392
642 0.9021186234328381
644 0.9011814371985097
647 0.9005036228265246
649 0.9008375865982594
650 0.9003642107322768
652 0.9008895686249541
655 0.8987936729387045
656 0.8985347362093175
659 0.8988113888472242
660 0.899223274958752
663 0.8981410422091645
665 0.8968476317870728
667 0.8966171554692021
669 0.89595998391451
671 0.896174384075365
672 0.8956136402346113
675 0.8942525038322652
676 0.8941549787939425
679 0.894433429006003
680 0.8934730947159429
683 0.8941103637687835
684 0.8934592601310957
687 0.8941816675297847
688 0.8934958508544869
691 0.891969892345942
693 0.8932941934224826
694 0.8929682514882579
697 0.8924235689733753
699 0.8927033332836415
700 0.8914042999508051
702 0.890693256951297
705 0.889844324381784
707 0.8899798811379661
708 0.8890530823265864
711 0.8891305515033205
712 0.8883222459882872
715 0.8885480235284043
717 0.8883455432931203
719 0.894190087860189
720 0.8929611869815871
722 0.8930335751117712
725 0.8922962393606535
727 0.8927782769670469
728 0.8927074941973765
730 0.8918374192554027
732 0.8921870450628487
735 0.8922441746122202
736 0.891001732866098
739 0.8908547155374369
740 0.8894841683820626
743 0.889199326698242
744 0.8894333334312595
747 0.8899240000969469
749 0.8883657600959775
751 0.8871501024950177
753 0.8873886014700675
754 0.8865847154553668
756 0.8867188683008131
758 0.8859776796178049
760 0.8856459028216268
762 0.8860134437934105
764 0.8849973093554764
766 0.8848543362619217
768 0.8850227928993025
770 0.8839445649703095
772 0.8838091193206065
774 0.8846210281274004
776 0.8839998178461265
779 0.8831258196676652
781 0.8833005614709886
783 0.8820945558562787
784 0.8819566102977159
787 0.8808520441947387
789 0.8806705237527914
791 0.8795248185152635
792 0.8793595703301109
794 0.8777379746268098
796 0.8777465948805416
799 0.8766421289317362
800 0.8769837076424188
803 0.8776968705659947
805 0.8770759018603348
806 0.8770711428417315
808 0.8758404314133141
810 0.875644027099181
813 0.8742055868281892
815 0.8742825309599073
817 0.8729457056503082
818 0.873492248593805
820 0.872577326107867
822 0.8739655528467882
824 0.8736838973183203
826 0.873189058345137
828 0.8732951677616857
831 0.8724062160840688
833 0.8726031539232281
834 0.8720821223839959
836 0.8707003011601558
839 0.8708472981485543
841 0.8705358251670687
842 0.870939466915398
844 0.8703120722462441
846 0.8696929515237816
848 0.8705080220085437
850 0.8702879417884583
853 0.8703610623705736
854 0.870924451746868
857 0.8699742072293992
858 0.8705384651571053
860 0.8705450805055343
862 0.8708486297004789
864 0.8699431434034741
866 0.8697297119694394
869 0.8691844148497451
870 0.8696975707012476
873 0.8694605949942352
875 0.869303989044293
876 0.8698549491538501
879 0.8689453996623117
881 0.8675329456656885
883 0.8674996162090316
884 0.8653156200469413
886 0.8655304638464718
888 0.8657791592080071
890 0.864933367615927
892 0.8649320339397677
895 0.86547471360037
897 0.8649459664643663
898 0.8652865067997226
901 0.8645886417317254
902 0.8661317553144082
904 0.8651554377612641
907 0.8664568833836515
908 0.866521314549815
910 0.8665461014043168
913 0.8651716403902736
915 0.8642429239863709
916 0.8650744947465072
918 0.8646387497990421
921 0.8649553623010517
922 0.8641488086780412
925 0.8633053205912607
927 0.8638472673853482
928 0.8630737947114947
931 0.8626780567643797
932 0.8630742761967359
934 0.8619795334347685
936 0.8619617381004209
938 0.8614171207194167
940 0.8618949495122225
943 0.8606330000171002
944 0.8608176700169292
946 0.8613574933167599
949 0.8609729183835924
950 0.8632811891997564
953 0.8628303773077588
955 0.8629490735346812
956 0.8620655827993344
958 0.8620789269713411
961 0.8616371377016278
962 0.8621447663246115
965 0.8610173186613653
966 0.8607541454747517
969 0.8596666040200042
971 0.8599969379798041
972 0.8584929686000061
974 0.858619038914006
976 0.8579358485248659
979 0.8573684900396172
981 0.858233805139221
982 0.8576334670878288
985 0.8578271324169506
986 0.8571848610927811
988 0.8574600124818533
991 0.8561794123570348
992 0.8558426182334644
995 0.8566271920511298
996 0.8556859201306185
999 0.8561570609293123
1000 0.8552804903200193
1002 0.8537596854168191
1005 0.8533110885626509
1007 0.8523369776770244
1008 0.8518456079002542
1011 0.8517121518212516
1013 0.8509560303030391
1015 0.8519054700000087
1017 0.8516084153000085
1018 0.8519143311470084
1021 0.8510041878355383
1023 0.850368145957183


==> iclr2026/plots/plot_bs16_phi2_uniprot.tex <==
0 1.213
1 1.214407
3 1.21625793
6 1.2173133507
7 1.219803217193
9 1.2197391850210701
12 1.2198387931708594
13 1.2204634052391508
15 1.2203427711867592
17 1.2200433434748914
20 1.2177899100401424
22 1.214977010939741
23 1.2140972408303436
25 1.21022726842204
27 1.2073899957378198
29 1.2049740957804416
31 1.2013423548226372
34 1.197675931274411
36 1.1951031719616667
38 1.1913801402420499
39 1.1878623388396294
42 1.1841807154512332
44 1.1797749082967208
46 1.1763151592137535
48 1.172047007621616
49 1.1692125375453999
52 1.1647374121699459
53 1.1599240380482465
56 1.156505797667764
57 1.1520817396910863
60 1.1485689222941755
62 1.1445402330712338
63 1.1414048307405213
66 1.137432782433116
67 1.133277454608785
70 1.1295666800626971
71 1.1261540132620702
74 1.1232034731294493
75 1.1195244383981549
77 1.1157401940141733
80 1.1127627920740317
82 1.1085151641532913
83 1.1050620125117585
85 1.1020033923866408
87 1.0975963584627744
89 1.0948553948781465
92 1.090976840929365
94 1.0866680725200715
95 1.0833463917948707
97 1.0797139278769219
99 1.0757477885981528
102 1.0730413107121712
104 1.0712628976050496
105 1.0681072686289992
108 1.0633231959427092
110 1.060430963983282
111 1.0568496543434494
113 1.0535041578000148
116 1.0497851162220146
117 1.0471142650597944
119 1.0447371224091966
121 1.0403957511851045
123 1.0372217936732535
126 1.0336095757365211
127 1.0309384799791559
130 1.0287980951793645
131 1.0259791142275707
133 1.023738323085295
136 1.0199619398544422
138 1.0167373204558976
139 1.0125959472513386
142 1.0103079877788252
143 1.0069239079010368
146 1.0041866688220265
147 1.000890802133806
149 0.998659894112468
151 0.9966072951713434
153 0.9932802222196299
156 0.9902264199974335
158 0.9878561557974592
160 0.9845675942394846
162 0.9820109182970898
163 0.9787588091141188
165 0.9752402210229776
168 0.9732578188127479
169 0.9699512406246205
172 0.9665147282183743
173 0.9646005809361905
175 0.9611665751268286
178 0.9585929093755603
179 0.9553649802818046
181 0.9535573304789866
183 0.9509787571741968
186 0.9501889696024548
187 0.9473440799064303
190 0.944912639107366
192 0.9421395127162924
194 0.9404351175891295
196 0.9378877664132381
197 0.9348548887491057
200 0.9332023398616147
202 0.9304113164629986
203 0.9282772032983686
205 0.9253404312653849
207 0.923743026952731
210 0.9212195966832037
212 0.9196404007163717
213 0.917274996709208
215 0.915871246742116
218 0.9126945342746948
220 0.9118075889319479
222 0.9090365130426284
224 0.9075891479122021
225 0.9047342564330801
228 0.9031259138687493
230 0.9009876547300618
231 0.8998907781827611
233 0.8974148704009334
236 0.895669721696924
237 0.8923970244799548
239 0.8901550542351553
241 0.8887835036928038
244 0.8869836686558757
246 0.885679831969317
247 0.8830110336496237
250 0.8815709233131275
251 0.8795112140799962
254 0.8770941019391962
256 0.8756391609198042
257 0.8735527693106061
260 0.8705112416175
261 0.8683251292013251
263 0.8657238779093118
266 0.8646336391302187
268 0.8617213027389166
269 0.8606890897115274
272 0.8594771988144121
274 0.857578426826268
276 0.8557786425580053
277 0.8535828561324252
280 0.8524040275711009
281 0.85029798729539
283 0.8495290074224361
285 0.8475847173482117
287 0.8458158701747296
290 0.8447237114729823
291 0.8431884743582525
294 0.84183158961467
296 0.8410962737185232
298 0.838695310981338
299 0.8370413578715246
301 0.8366719442928093
303 0.8349502248498812
306 0.8334847226013824
308 0.8323608753753685
310 0.8303122666216148
311 0.8288551439553987
313 0.8267425925158447
316 0.8258131665906862
317 0.8241470349247794
319 0.8231485645755315
321 0.8225560789297761
323 0.8207425181404783
325 0.8195840929590734
327 0.8171362520294827
330 0.8166718895091879
332 0.814394170614096
333 0.8131972289079551
336 0.8111352566188755
338 0.8106539040526868
340 0.8091143650121599
341 0.8085422213620383
344 0.807734799148418
345 0.8059734511569338
348 0.8045007166453644
349 0.8038567094789107
351 0.8020611423841216
353 0.8011995309602804
355 0.7997665356506776
358 0.7990218702941707
360 0.797859651591229
361 0.7968550550753167
364 0.7958045045245635
366 0.7952534594793179
368 0.7932359248845248
370 0.7920195656356794
371 0.7904283699793226
373 0.7897180862795294
375 0.787598905416734
377 0.7871869163625668
379 0.785951047198941
382 0.7841195367269517
383 0.7829863413596821
385 0.7817434779460853
387 0.7813120431666245
389 0.7792759227349583
391 0.7775571635076087
394 0.7765885918725326
395 0.7749397059538073
398 0.7744543088942694
399 0.7735037658053266
401 0.7730447281472733
404 0.7712272808658005
406 0.7700350080571424
408 0.768295657976571
409 0.7670347013968053
412 0.7669623543828372
413 0.7658987308390088
415 0.7640837435306187
417 0.7627209060953125
419 0.7612036970343593
421 0.7607096600640156
424 0.7605115634633755
425 0.7594424478287417
428 0.7581910233504543
429 0.7575461131169497
431 0.7570426519857802
433 0.7561202254659224
435 0.7558770232112632
438 0.7553592529791505
439 0.754593660449359
442 0.7522197238448654
443 0.7514375266064166
446 0.7500991513403524
448 0.7489861598269488
449 0.7483262982286794
451 0.7486240352463925
453 0.7489377948939286
455 0.7476994169449893
458 0.7479114227755393
460 0.7463883085477839
462 0.7455304254623061
463 0.745218121207683
465 0.7443549399956062
468 0.7438733905956502
470 0.7424896566896937
472 0.7418267601227968
474 0.7406604925215688
475 0.7411978875963531
478 0.7402559087203895
480 0.7388743496331857
481 0.7378916061368538
484 0.7364226900754852
485 0.7357234631747304
488 0.7345092285429831
490 0.7347061362575533
491 0.7336540748949778
493 0.7324535341460281
495 0.7316679988045678
498 0.7310943188165222
500 0.7295383756283569
502 0.7281829918720732
504 0.7272341619533526
506 0.7256738203338191
507 0.7263780821304809
510 0.725630301309176
513 0.7248719982960843
515 0.7232412783131235
516 0.7221858655299922
519 0.7217850068746923
521 0.7206311568059452
523 0.7192198452378857
524 0.7177466467855069
526 0.7176301803176518
528 0.7168138785144753
531 0.7171537397293305
532 0.7159492023320373
534 0.7158507103087169
536 0.7143252032056298
538 0.7141059511735734
541 0.7133668916618378
543 0.7131742227452194
544 0.7132664805177672
546 0.7124928157125895
548 0.7123728875554636
550 0.7125471586799089
553 0.7117676870931098
554 0.7115640102221786
557 0.7103213701199569
559 0.7098891564187573
560 0.7082172648545697
563 0.706803092206024
565 0.7064350612839638
567 0.7061307106711242
569 0.705043403564413
571 0.7051289695287689
573 0.7047816798334813
575 0.7030648630351465
576 0.701231214404795
579 0.701350902260747
581 0.7006623932381396
583 0.7011177693057582
584 0.7010625916127006
586 0.7015579656965736
589 0.6999873860396079
590 0.6995755121792118
592 0.6986547570574198
594 0.6972502094868456
597 0.6967207073919771
598 0.6960995003180573
601 0.6948315053148767
602 0.695339190261728
604 0.6941457983591107
607 0.6945593403755196
608 0.6937317469717643
611 0.6939534295020467
613 0.6923548952070263
615 0.692349346254956
616 0.6914188527924064
619 0.6908746642644824
620 0.6897789176218375
623 0.6895851284456191
624 0.6883422771611629
627 0.6887878543895514
628 0.6884219758456559
630 0.6875977560871993
632 0.6865057785263273
634 0.6854917207410641
637 0.6845748035336535
639 0.684298055498317
640 0.6834080749433338
643 0.6836699941939004
644 0.6827032942519614
646 0.6826362613094418
649 0.6820698986963474
651 0.6822521997093839
652 0.68071467771229
655 0.6807335309351671
656 0.6792081956258155
658 0.6792171136695573
661 0.6792089425328617
663 0.677789853107533
664 0.6781609545764576
667 0.6770633450306931
668 0.6769577115803862
670 0.6759391344645823
673 0.6763827431199364
675 0.675260915688737
676 0.6741243065318496
678 0.6739730634665311
680 0.6736263328318658
683 0.6744760695035471
684 0.6734033088085116
686 0.6728602757204265
688 0.6719036729632223
691 0.67216763623359
692 0.670976959871254
694 0.6713151902725416
697 0.6723080383698162
698 0.671529957986118
700 0.6711886584062569
702 0.6710207718221943
705 0.6699725641039724
706 0.6701938384629327
708 0.6694519000783034
710 0.6693623810775203
712 0.6702037572667451
714 0.6697177196940777
717 0.6685785424971369
718 0.6687967570721656
720 0.6690537895014439
722 0.6693162516064295
725 0.6682990890903652
726 0.6684720981994615
729 0.666584377217467
730 0.6667785334452923
732 0.6671487481108394
734 0.666435260629731
736 0.6666799080234338
739 0.6669101089431995
740 0.6663510078537674
743 0.6659354977752298
744 0.6661301427974775
746 0.6669048413695027
749 0.6661997929558077
751 0.6659477950262496
752 0.6651183170759871
754 0.6653501339052272
757 0.6653666325661749
758 0.6645229662405131
761 0.663505736578108
763 0.6634946792123269
765 0.6634627324202036
766 0.6620651050960016
769 0.6607274540450416
770 0.6602421795045912
773 0.6609217577095453
774 0.6598415401324499
777 0.6611221247311253
778 0.6599869034838141
780 0.6597410344489759
782 0.6597006241044862
784 0.6602956178634413
786 0.6596166616848069
789 0.6578944950679589
791 0.6585155501172794
793 0.6572023946161066
794 0.6573893706699455
796 0.657722476963246
799 0.6575002521936135
800 0.6560682496716774
802 0.6553435671749606
805 0.655309131503211
806 0.6541910401881789
808 0.6535441297862971
811 0.6535416884884341
813 0.6527792716035498
814 0.6526464788875143
817 0.6511470140986391
818 0.6510205439576526
821 0.6501363385180762
822 0.6500989751328954
824 0.6494509853815664
827 0.6490004755277508
829 0.6475134707724732
830 0.6470583360647485
833 0.646549752704101
835 0.6475042551770599
836 0.6464942126252894
838 0.6466762704990364
841 0.6459365077940461
843 0.6449171427161057
845 0.6452619712889446
846 0.6447523515760551
848 0.6449898280602946
850 0.6438339297796917
853 0.6437045904818948
855 0.6424015445770758
857 0.642425529131305
859 0.642076273839992
861 0.642918511101592
863 0.6427523259905761
865 0.6429358027306703
867 0.6416474447033635
869 0.6425279702563299
870 0.6422846905537666
873 0.6428688436482289
875 0.6417291552117467
876 0.6411718636596292
879 0.6411171450230329
881 0.6404079735728025
883 0.6406708938370745
885 0.6395681848987038
886 0.6392025030497167
888 0.6385664780192195
891 0.6387558132390273
892 0.6382142551066371
894 0.6382961125555707
896 0.6374821514300151
899 0.637980329915715
901 0.6374005266165579
903 0.6376245213503923
905 0.6381452761368884
907 0.6375688233755195
909 0.6369991351417642
911 0.6373361437903465
913 0.6361987823524431
914 0.6360377945289186
917 0.6350084165836294
918 0.6346853324177931
921 0.6341204790936151
923 0.634377274302679
925 0.6339645015596522
926 0.6336318565440557
928 0.6343835379786151
930 0.634313702598829
933 0.6339135655728407
935 0.6332584299171123
937 0.6336018456179412
939 0.6332718271617618
940 0.6331571088901441
942 0.6324865378012426
944 0.6326236724232301
947 0.6334504356989978
948 0.6342559313420079
950 0.6333623720285878
953 0.6328147483083019
955 0.6336396008252188
957 0.6329132048169666
959 0.6325040727687969
960 0.6339650320411089
962 0.6339303817206978
965 0.6330320779034909
966 0.6334647571244559
968 0.6330951095532114
970 0.6336251584576792
972 0.6341759068731023
974 0.6345991478043713
976 0.6339401563263276
979 0.6332287547630643
980 0.6334104672154337
982 0.6331153625432794
984 0.6336932089178466
986 0.6331922768286681
989 0.6331033540603814
991 0.6320093205197777
992 0.6323952273145799
995 0.6325412750414341
996 0.6311768622910198
999 0.6317860936681096
1001 0.6322272327314284
1002 0.6315869604041141
1005 0.6308380908000729
1007 0.6311927098920721
1009 0.6307987827931514
1011 0.6301867949652199
1013 0.6300289270155678
1014 0.629653637745412
1017 0.630596101367958
1018 0.6300991403542783
1021 0.6296501489507355
1023 0.6287756474612282

